Detecting and Defending Against Adversarial Attacks on Automatic Speech Recognition via Diffusion Models

Automatic speech recognition (ASR) systems are known to be vulnerable to adversarial attacks. This paper addresses detection and defence against targeted white-box attacks on speech signals for ASR systems. While existing work has utilised diffusion models (DMs) to purify adversarial examples, achieving state-of-the-art results in keyword spotting tasks, their effectiveness for more complex tasks such as sentence-level ASR remains unexplored. Additionally, the impact of the number of forward diffusion steps on performance is not well understood. In this paper, we systematically investigate the use of DMs for defending against adversarial attacks on sentences and examine the effect of varying forward diffusion steps. Through comprehensive experiments on the Mozilla Common Voice dataset, we demonstrate that two forward diffusion steps can completely defend against adversarial attacks on sentences. Moreover, we introduce a novel, training-free approach for detecting adversarial attacks by leveraging a pre-trained DM. Our experimental results show that this method can detect adversarial attacks with high accuracy.

==> P7/8Acknowledgement.tex <==

%\section{Acknowledgement}

%\noindent We thank the authors of the Mozilla Common Voice dataset for making their datasets publicly available. %Furthermore, we thank Nicholas Carlini and David Wagner for providing code used and we thank Baidou Deep Speech for making Deep Speech publicly available.

==> P7/guide.tex <==
\section{Guide}

\noindent Dear readers of this paper :)
Greetings from the dark side of speech recognition.
We have worked hard on this paper - so sit back and enjoy the ride (even if it is a bit bumpy).

\bigskip
Comments before reading 
\begin{itemize}
    \item The results are not completely finished as we do not have any results for sentences and, therefore, will not be commented on in the result nor the discussion. Specifically, the results in Table 1 for WB-S, WB-M and WB-L and in Table 2 for WB-S, WB-M and WB-L are not finished.
    \item Throughout the article there are a few places where we mention the sentences e.g. in the abstract and in Section III-B See if you can ignore this. 
    %, and not to flex but since no one have done what we do, we really don't have a clue what the results should be. We really are amazing.
    \item We do not have a conclusion, since our project primarily is based on the extension to sentences.

\end{itemize}

\bigskip

Thank you for reading - hope you have fun.
\newpage

==> Preamble.tex <==
% \usepackage{graphicx} % Required for inserting images

% \usepackage{fancyhdr}
% \usepackage[explicit]{titlesec}

% \bibliographystyle{IEEEtran}			% Udseende af litteraturlisten (Harvard-metoden - skift til fx 'plain' for tal)

% \usepackage[T1]{fontenc}% optional T1 font encoding

% *** CITATION PACKAGES ***
%
% \usepackage{cite}
% cite.sty was written by Donald Arseneau
% V1.6 and later of IEEEtran pre-defines the format of the cite.sty package
% \cite{} output to follow that of the IEEE. Loading the cite package will
% result in citation numbers being automatically sorted and properly
% "compressed/ranged". e.g., [1], [9], [2], [7], [5], [6] without using
% cite.sty will become [1], [2], [5]--[7], [9] using cite.sty. cite.sty's
% \cite will automatically add leading space, if needed. Use cite.sty's
% noadjust option (cite.sty V3.8 and later) if you want to turn this off
% such as if a citation ever needs to be enclosed in parenthesis.
% cite.sty is already installed on most LaTeX systems. Be sure and use
% version 5.0 (2009-03-20) and later if using hyperref.sty.
% The latest version can be obtained at:
% http://www.ctan.org/pkg/cite
% The documentation is contained in the cite.sty file itself.


% *** PDF, URL AND HYPERLINK PACKAGES ***
%
% \usepackage{url}
% url.sty was written by Donald Arseneau. It provides better support for
% handling and breaking URLs. url.sty is already installed on most LaTeX
% systems. The latest version and documentation can be obtained at:
% http://www.ctan.org/pkg/url
% Basically, \url{my_url_here}.


% %%%%%%%%%%%%%%%%%%%% Title %%%%%%%%%%%%%%%%%%%%
% \usepackage{titling} % Required for customizing the title section

% \setlength{\droptitle}{-7\baselineskip} % Move the title up

% \pretitle{\begin{center}\Large\bfseries\MakeUppercase} % Article title pre-formatting
% % \pretitle{\begin{center}\huge\bfseries} % Article title pre-formatting
% \posttitle{\end{center}} % Article title post-formatting

% % \patchcmd{\maketitle}{plain}{empty}{}{} % Set the headers and footers style for the first page to empty
\newcommand{\norm}[1]{\left\lVert#1\right\rVert}
% \usepackage{algpseudocode}
% \usepackage[section]{algorithm}
% \usepackage{algorithm2e}
% \RestyleAlgo{ruled}

% %%%%%%%%%%%%%%%%%%%% Sections %%%%%%%%%%%%%%%%%%%%
% \usepackage{titlesec} % Required for modifying sections
% \titleformat
% 	{\section} % Section type being modified
% 	[block] % Section layout type, can be: hang, block, display, runin, leftmargin, rightmargin, drop, wrap, frame
% 	{\normalsize\bfseries\centering} % Text formatting of the whole section, i.e. label and title
% 	{\thesection.} % Section label (e.g. number) and its formatting
% 	{0.5em} % Horizontal space between the section label and title
% 	{\MakeUppercase} % Code before the section title
% 	[] % Code after the section title



% %%%%%%%%%%%%%%%%%%%% Subsections %%%%%%%%%%%%%%%%%%%%

% \titleformat
% 	{\subsection} % Section type being modified
% 	[block] % Section layout type, can be: hang, block, display, runin, leftmargin, rightmargin, drop, wrap, frame
% 	{\normalsize\bfseries} % Text formatting of the whole section, i.e. label and title
% 	{\thesubsection.} % Section label (e.g. number) and its formatting
% 	{0.5em} % Horizontal space between the section label and title
% 	{} % Code before the section title
% 	[] % Code after the section title

% \usepackage[colorlinks,allcolors=blue]{hyperref}
% \usepackage{hyperref}


\usepackage{balance}                % Balances the columns of the last page
\usepackage{dirtytalk} %benytte \say til at lave pæne anførselstegn
\hyphenation{op-tical net-works semi-conduc-tor}% correct bad hyphenation here
% ¤¤ Matematik mm. ¤¤
% \usepackage{amsmath,amssymb,stmaryrd}		% Avancerede matematik-udvidelser
% \usepackage{mathtools}						% Andre matematik- og tegnudvidelser
% \mathtoolsset{showonlyrefs, showmanualtags} %removes equation numbering
% \usepackage{textcomp}                 		% Symbol-udvidelser (fx promille-tegn med \textperthousand)
\usepackage{siunitx}						% Flot og konsistent praesentation af tal og enheder med \si{enhed} og \SI{tal}{enhed}
\sisetup{output-decimal-marker = {.}}		% Opsaetning af \SI og decimalseparator
%\usepackage[version=3]{mhchem} 			% Kemi-pakke til flot og let notation af formler, fx \ce{Fe2O3}
%\usepackage{rsphrase}						% Kemi-pakke til RS-saetninger, fx \rsphrase{R1}
\usepackage[official]{eurosym} 
\let\EUR\undefined
%Possibility to highlight text
% \usepackage{color,soul}
\usepackage{soul}
% \usepackage{bm}

\makeatletter
\newcommand*{\bigs}[1]{{\hbox{$\left#1\vbox to10\p@{}\right.\n@space$}}}
\makeatother

\makeatletter
\newcommand*{\biggs}[1]{{\hbox{$\left#1\vbox to17\p@{}\right.\n@space$}}}
\makeatother

% \usepackage[
%     protrusion=true,
%     activate={true,nocompatibility},
%     final,
%     tracking=true,
%     kerning=true,
%     spacing=true,
%     factor=1100]{microtype}
% \SetTracking{encoding={*}, shape=sc}{40}


\usepackage[english]{babel}
\usepackage{blindtext}

\usepackage{tikz}  %Pakke til plot af funktioner og grafer
\usetikzlibrary{decorations.pathreplacing,calligraphy}
\usepackage[framemethod=tikz]{mdframed}
% \usepackage[dvipsnames]{xcolor}
\usetikzlibrary{shapes.geometric, arrows, arrows.meta}
% \usepackage{subcaption}
\usepackage{graphicx}
\usepackage{float}
\usepackage{booktabs}
\usepackage{multirow}
\usepackage{dblfloatfix}
\DeclareSIUnit[quantity-product = ]\percent{\char`\%}
\usepackage{comment}
\usetikzlibrary{decorations.text}
\usetikzlibrary{shapes.geometric, arrows}
\usetikzlibrary{positioning}

%\newcommand{\audiopure}{{\small{\fontfamily{qhv}\selectfont AudioPure}} }
\newcommand{\audiopure}{Audio\-Pure }


% *** Do not adjust lengths that control margins, column widths, etc. ***
% *** Do not use packages that alter fonts (such as pslatex).         ***
% There should be no need to do such things with IEEEtran.cls V1.6 and later.
% (Unless specifically asked to do so by the journal or conference you plan
% to submit to, of course. )


\def\,{\mskip\thinmuskip} \def\!{\mskip-\thinmuskip}
\def\,{\mskip\thickmuskip} \def\;{\mskip+\thickmuskip}




% Fra IEEE
% \IEEEoverridecommandlockouts
% The preceding line is only needed to identify funding in the first footnote. If that is unneeded, please comment it out.
\usepackage{cite}
\usepackage{spconf,amsmath,amssymb,amsfonts,mathtools}
\usepackage{algorithmic}
\usepackage{graphicx}
\usepackage{textcomp}
\usepackage{xcolor}
\def\BibTeX{{\rm B\kern-.05em{\sc i\kern-.025em b}\kern-.08em
    T\kern-.1667em\lower.7ex\hbox{E}\kern-.125emX}}


% Egne tilføjelser
\usepackage{bm}
\usepackage{comment}
\newcommand\abs[1]{\left|#1\right|}
\usepackage{pifont} % Checkmark
\makeatletter
\newcommand*\bigcdot{\mathpalette\bigcdot@{.5}}
\newcommand*\bigcdot@[2]{\mathbin{\vcenter{\hbox{\scalebox{#2}{$\m@th#1\bullet$}}}}}
\makeatother
% \DeclareSIUnit[quantity-product = ]\percent{\char`\%}
\usepackage{tikz}  %Pakke til plot af funktioner og grafer
\usepackage{url}

% \usepackage{tikzpeople}
% \usetikzlibrary{calc}
% \usetikzlibrary{decorations.pathreplacing,decorations.markings,shapes.geometric}
% \tikzset{naming/.style={align=center,font=\small}}
% \tikzset{antenna/.style={insert path={-- coordinate (ant#1) ++(0,0.25) -- +(135:0.25) + (0,0) -- +(45:0.25)}}}
% \tikzset{station/.style={naming,draw,shape=dart,shape border rotate=90, minimum width=10mm, minimum height=10mm,outer sep=0pt,inner sep=3pt}}
% %\tikzset{mobile/.style={naming,draw,shape=rectangle,minimum width=15mm,minimum height=7.5mm, outer sep=0pt,inner sep=3pt}}
% \tikzset{mobile/.style={naming,draw,shape=rectangle,minimum width=12mm,minimum height=6mm, outer sep=0pt,inner sep=3pt}}
% \tikzset{radiation/.style={{decorate,decoration={expanding waves,angle=90,segment length=4pt}}}}

% \tikzset{axis/.style={thick,-latex}}
% \tikzset{vec/.style={thick,blue}}
% \tikzset{univec/.style={thick,red,-latex}}
% \usetikzlibrary{patterns}


==> Tabeller/Overview.tex <==
    \begin{tabular}{@{}l|c|c@{}}
        \toprule
        Dataset    & GSC v$0.01$       & MCV         \\\hline
        Utterances & Keywords        & Sentences   \\\hline
        Attack     & Black-box (Alzantot)       & White-box (C\&W)   \\\hline
        Classifier & Keyword spotter & Deep Speech \\\hline
        \bottomrule
    \end{tabular}

==> Tabeller/PurifyKeywords.tex <==
    \begin{tabular}{@{}l|cccc@{}}
        \toprule
        Defence & C-KS           & BB             & C-DS           & WB             \\ \hline
        None                                                  
        & \textbf{93.00} & 9.83           & \textbf{65.00} & 1.44           \\
        \textbf{Purifier} $n^{\star}=1$ 
        & 92.00$\pm$100          & 64.22($\pm$100)          & 53.50($\pm$100)           & \textbf{49.89}($\pm$100) \\
        \textbf{Purifier} $n^{\star}=2$ 
        & 89.00          & 73.17          & 48.50          & 42.50          \\
        \textbf{Purifier} $n^{\star}=3$ 
        & 88.50          & 76.44          & 46.50          & 37.67          \\
        \textbf{Purifier} $n^{\star}=4$ 
        & 82.00          & 77.06          & 37.50          & 35.61          \\
        \textbf{Purifier} $n^{\star}=5$ 
        & 80.50          & \textbf{77.33} & 30.50          & 31.50          \\
        \bottomrule

    \end{tabular}

==> Tabeller/PurifySentences.tex <==
    \begin{tabular}{@{}l|cccccc@{}}
        \toprule
        Defence    & C-DS-S         & WB-S  & C-DS-M  & WB-M  & C-DS-L   & WB-L    \\ \hline
        None                                                  
        & \textbf{78.00} & 19.41  & \textbf{86.01}       & 20.58     & \textbf{86.07}       & 24.67\\
        \textbf{Purifier} $n^{\star}=1$ 
        & 71.91($\pm$1.04)          & 41.97($\pm$100) & 75.93($\pm$0.42)       & 34.70($\pm$100)& 73.62($\pm$100)       & 36.00($\pm$100)\\
        \textbf{Purifier} $n^{\star}=2$ 
        & 64.71($\pm$0.48)          & 45.12 & 67.21($\pm$0.24)       & 40.23     & 65.50       & 40.29\\
        \textbf{Purifier} $n^{\star}=3$ 
        & 58.91($\pm$0.45)          & 46.40 & 61.05($\pm$0.09)       & 44.50    & 57.76       & 44.07\\
        \textbf{Purifier} $n^{\star}=4$ 
        & 54.61($\pm$0.42)          & \textbf{46.70} & 55.70($\pm$0.38)       & \textbf{46.16}    & 52.60       & \textbf{45.31}\\
        \textbf{Purifier} $n^{\star}=5$ 
        & 50.29($\pm$2.07)          & 45.73 & 51.02       & 45.17    & 47.12       & 44.34\\
        \bottomrule

    \end{tabular}

==> billeder/DDPM2.tex <==
\begin{tikzpicture}[trim left=-8mm]
    % Grid
     %\draw[step=0.02cm,gray!20,very thin] (4,-1.5) grid (8,0);

    % Cirkler
    \node[circle, draw, minimum size=0.76cm](x0){\footnotesize$\bm{x}_0$};
    \node[circle, draw, minimum size=0.76cm, xshift=-0.15cm](x1)[right = of x0]{\footnotesize$\bm{x}_1$};
    \node[circle, draw, minimum size=0.76cm, xshift=-0.15cm](x2) [right = of x1] {\footnotesize$\bm{x}_2$};
    
    \node[circle, inner sep=0pt, draw, minimum size=0.76cm, xshift=-0.5cm](xT-1)[right = of x2]{\footnotesize$\bm{x}_{T-1}$};
    \node[circle, draw, minimum size=0.76cm, xshift=-0.1cm](xT) [right = of xT-1] {\footnotesize$\bm{x}_T$};

    % Pile mellem cirkler
    \draw[arrows = {-Latex[width=3pt, length=4pt]}] (x0) edge [bend left]  node[sloped, above] {\footnotesize$q(\bm{x}_1\vert \bm{x}_0)$} (x1);
    \draw[arrows = {-Latex[width=3pt, length=4pt]}] (x1) edge [bend left] node[above]{\footnotesize$q(\bm{x}_2\vert \bm{x}_1)$} (x2);
    \draw[arrows = {-Latex[width=3pt, length=4pt]}] (x2) edge [bend left] node[below]{\footnotesize$p_{\bm{\theta}}(\bm{x}_1\vert \bm{x}_2)$} (x1);
    \draw[arrows = {-Latex[width=3pt, length=4pt]}] (x1) edge [bend left] node[below]{\footnotesize$p_{\bm{\theta}}(\bm{x}_0\vert \bm{x}_1)$} (x0);

    \draw[arrows = {-Latex[width=3pt, length=4pt]}] (xT-1) edge [bend left] node[above, xshift=-0.0cm]{\footnotesize$q(\bm{x}_T\vert \bm{x}_{T-1})$} (xT);
    \draw[arrows = {-Latex[width=3pt, length=4pt]},] (xT) edge [bend left] node[below, xshift=0.08cm]{\footnotesize$p_{\bm{\theta}}(\bm{x}_{T-1}\vert \bm{x}_T)$} (xT-1);

    % Pile i midten
    \draw[arrows = {-Latex[width=3pt, length=4pt]}] (3.7+0.18-0.12-0.025-0.1,0.4) -- (4.2+0.18-0.12-0.025-0.1,0.4) node[above, pos=0.5]{};
    \draw[arrows = {-Latex[width=3pt, length=4pt]}] (4.2+0.18-0.12-0.025-0.1,-0.4) -- (3.7+0.18-0.12-0.025-0.1,-0.4) node[below, pos=0.5]{};
    \node at (4+0.18-0.125-0.025-0.1,0) {$\cdots$};

    % Billeder
    \node at (0,1.3) {\includegraphics[width=1.7cm]{billeder/x0a.pdf}};
    \node at (1.65+0.06-0.05-0.05,-1.3) {\includegraphics[width=1.7cm]{billeder/x1a.pdf}};
    \node at (3.3+0.12-0.1-0.1,1.3) {\includegraphics[width=1.7cm]{billeder/x2a.pdf}};
    \node at (4.6+0.18-0.15-0.05-0.1,-1.3) {\includegraphics[width=1.7cm]{billeder/xT_1a.pdf}};
    \node at (6.25+0.24-0.2-0.1,1.3) {\includegraphics[width=1.7cm]{billeder/xTa.pdf}};

    % Prikker
    \draw[dotted, blue, thick] (0,1) -- (0,0.55);
    \draw[dotted, blue, thick] (1.65+0.06-0.05-0.05,-1) -- (1.65+0.06-0.05-0.05,-0.55);
    \draw[dotted, blue, thick] (3.3+0.12-0.1-0.1,1) -- (3.3+0.12-0.1-0.1,0.55);
    \draw[dotted, blue, thick] (4.6+0.18-0.15-0.05-0.1,-1) -- (4.6+0.18-0.15-0.05-0.1,-0.55);
    \draw[dotted, blue, thick] (6.25+0.24-0.2-0.1,1) -- (6.25+0.24-0.2-0.1,0.55);


    \node at (-0.4,0.583) {\footnotesize{$q(\bm{x}_0)$}};
    \node at (6.9-0.05,-0.584){\footnotesize{$p(\bm{x}_T)$}};
    % \node at (6.98,-0.584){\footnotesize{$p(\bm{x}_T)$}};

    %7.38
\end{tikzpicture}
